MQM-Chat: Multidimensional Quality Metrics for Chat Translation

The complexities of chats pose significant challenges for machine translation models. Recognizing the need for a precise evaluation metric to address the issues of chat translation, this study introduces Multidimensional Quality Metrics for Chat Translation (MQM-Chat). Through the experiments of five models using MQM-Chat, we observed that all models generated certain fundamental errors, while each of them has different shortcomings, such as omission, overly correcting ambiguous source content, and buzzword issues, resulting in the loss of stylized information. Our findings underscore the effectiveness of MQM-Chat in evaluating chat translation, emphasizing the importance of stylized content and dialogue consistency for future studies.

==> table/mistranslation_relabeled_comparison_1.tex <==
\begin{table*}[ht]
\centering
\small
\tabcolsep=3pt
\begin{tabular}{@{}llcccccccc@{}}
\toprule
&&&
\multicolumn{3}{c}{\textit{\textbf{zh$\Rightarrow$en}}} && \multicolumn{3}{c}{\textit{\textbf{ja$\Rightarrow$en}}} \\ 
 \textbf{Data} & \textbf{Model} && \textbf{Mistrans. \#} & \textbf{Re-labeled (\%)} & \textbf{Chat-spec (\%)} && \textbf{Mistrans. \#} & \textbf{Re-labeled (\%)} & \textbf{Chat-spec (\%)} \\
\cmidrule{1-2}
\cmidrule{4-6}
\cmidrule{8-10}
Short 
&\textbf{GPT-4} && 160 & \;\,48 (30.00\%) & \;\,29 (18.12\%) && \;\,88 & \;\,44 (50.00\%) & \;\,27 (30.68\%) \\
&\textbf{LLaMA3} && 315 & 143 (45.40\%) & \;\,90 (28.57\%) && 293 & 228 (77.82\%) & 120 (40.96\%) \\
&\textbf{DeepL} && 426 & 210 (49.30\%) & 136 (31.92\%) && 316 & 197 (62.34\%) & \;\,95 (30.06\%) \\
&\textbf{NMT} && 599 & 272 (45.41\%) & \;\,76 (12.69\%) && 467 & 390 (83.51\%) & 198 (42.40\%) \\
\cmidrule{1-2}
\cmidrule{4-6}
\cmidrule{8-10}
Long
&\textbf{GPT-4} && 109 & \;\,22 (20.18\%) & \;\,\;\,9 (\;\,8.26\%) && \;\,29 & \;\,\;\,9 (31.03\%) &\;\,\;\,4 (13.79\%) \\
&\textbf{LLaMA3} && 253 & \;\,53 (20.95\%) & \;\,20 (\;\,7.91\%) && \;\,83 & \;\,36 (43.37\%) & \;\,11 (13.25\%) \\
&\textbf{DeepL} && 619 & 203 (32.70\%) & \;\,93 (15.02\%) && 175 & \;\,66 (37.71\%) & \;\,21 (12.00\%) \\
&\textbf{NMT} && 957 & 250 (26.12\%) & 120 (12.54\%) && 390 & 237 (60.77\%) & \;\,73 (18.72\%) \\ \bottomrule
\end{tabular}
\caption{The percentage of errors labeled as \textit{Mistranslation} 
in standard MQM auto annotations being re-labeled in the MQM-Chat human annotations. \textbf{Mistrans.\#} represents the number of errors classified as \textit{Mistranslations} in standard MQM auto annotations. \textbf{Re-labeled (\%)} states the number and percentage of \textit{Mistranslations} being re-labeled into other error types in the MQM-Chat human annotations. \textbf{Chat-spec (\%)} indicates the percentage of \textit{Mistranslations} re-labeled specifically to chat-specific error types in the MQM-Chat metric, such as \textit{Ambiguity}, \textit{Buzzword Issues}, and \textit{Dialogue Inconsistency}.}
\label{tab:mistranslation_relabeled_comparison}
\end{table*}


==> table/system_level_pairwise_pearson.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\centering
\small
\begin{tabular}{@{}lc@{}}
\toprule
& \textbf{MQM-Chat Auto Annotations} \\ \midrule
\textbf{Pairwise Acc.}  & 79.17\% \\
\textbf{Pearson Corr.}  & 0.774 \\
\textbf{p-value}        & 0.00044 \\ \bottomrule
\end{tabular}
\caption{The system-level pairwise accuracy, the Pearson correlation, and the Pearson p-value of MQM-Chat auto annotations compared to the MQM-Chat human annotations, based on the overall quality scores.}
\label{tab:system_level_pairwise_pearson}
\end{table}

==> trash/few_shot_examples.tex <==
\begin{figure*}[hbt]{
\begin{lstlisting}

Chinese source:
王小明昨天去故宫了
谁？是那个微信昵称叫全垒打的吗？
English translation: 
Ong Xiaoming went to Gu palace yesterday
Who? The one whose WeChat nickname is Whole Round Hit?
MQM annotations:
Critical:
no-error
Major:
accuracy/mistranslation - "Ong Xiaoming"
accuracy/mistranslation - "Gu palace"
accuracy/mistranslation - "Whole Round Hit"
Minor:
no-error

Chinese source:
你造吗？我昨天看见海伦了！
袜喔、上次见她还是去年冬天呢
English translation:
You know what? I saw Helen yesterday!
Socks. Last time I saw her was last winter.
MQM annotations:
Critical:
accuracy/mistranslation - "Socks."
Major:
no-error
Minor:
no-error

Chinese source: 
给力啊！你是高中生吗？
草啊www为什么这么问？五杀必须年轻吗
不是不是，就是问问，爱你么么哒
English translation:
Give it a shot! Are you a student?
Grass www Why do you ask? Do you have to be young to get five kills?
No, no, no. Just asking. Love you kissing around.
MQM annotations:
Critical:
accuracy/mistranslation - "Grass"
style/awkward - "kissing around"
Major:
fluency/inconsistency - "Do you have to be young to get five kills?"
Minor:
accuracy/mistranslation - "Give it a shot!"
accuracy/mistranslation - "student"

Japanese source:
知ってｒ？昨日、ヘレンとあったよ！
ワウ、去年の冬いらいひざしぶりにヘレンと出会ったね
English source:
You know what? I saw Helen yesterday!
Wow, you've been knee-deep in Helen since last winter!
MQM annotations:
Critical:
accuracy/mistranslation - "knee-deep in Helen"
Major:
no-error
Minor:
no-error

Japanese source: 
バ美肉おじさんになった草wwww
えっwwww高校生じゃないの
English source:
Uncle Bami Meat became Grass
Awww, you are not a student?
MQM annotations:
Critical:
accuracy/mistranslation - "Uncle Bami Meat became Grass"
Major:
no-error
Minor:
style/awkward - "Awww"
accuracy/mistranslation - "student"

Japanese source: 
昨日ハマスタに行った？
行った！！！！めっちゃスゴなホームランだったな！
English source:
Did you go to Hamasta yesterday?
You did！！！！ That was a really awesome whole earth hit!
MQM annotations:
Critical:
fluency/inconsistency - "You"
Major:
accuracy/mistranslation - "Hamasta"
accuracy/mistranslation - "whole earth hit"
Minor:
no-error

Chinese source:
王小明昨天去故宫了
谁？是那个微信昵称叫全垒打的吗？
English source:
Ong Xiaoming went to Gu palace yesterday
Who? The one whose WeChat nickname is Whole Round Hit?
MQM annotations:
Major:
no-error
Minor:
Terminology or Proper Noun Issues - "Ong Xiaoming"
Terminology or Proper Noun Issues - "Gu palace"
Terminology or Proper Noun Issues - "Whole Round Hit"
Neutral:
no-error

Chinese source:
你造吗？我昨天看见海伦了！
袜喔、上次见她还是去年冬天呢
English source:
You know what? I saw Helen yesterday!
Socks. Last time I saw her was last winter.
MQM annotations:
Major:
Ambiguity and Disambiguation - "Socks."
Minor:
no-error
Neutral:
Ambiguity and Disambiguation - "You know what?"

Chinese source:
给力啊！你是高中生吗？
草啊www为什么这么问？五杀必须年轻吗
不是不是，就是问问，爱你么么哒
English source:
Give it a shot! Are you a student?
Grass www Why do you ask? Do you have to be young to get five kills?
No, no, no. Just asking. Love you kissing around.
MQM annotations:
Major:
Buzzword or Loanword Issues - "Grass"
Buzzword or Loanword Issues - "kissing around"
Minor:
Dialogue Inconsistency - "Do you have to be young to get five kills?"
Neutral:
Buzzword or Loanword Issues - "Give it a shot"
Mistranslation - "student"

Japanese source:
知ってｒ？昨日、ヘレンとあったよ！
ワウ、去年の冬いらいひざしぶりにヘレンと出会ったね
English source:
You know what? I saw Helen yesterday!
Wow, you've been knee-deep in Helen since last winter!
MQM annotations:
Major:
Ambiguity and Disambiguation - "knee-deep in Helen"
Minor:
no-error
Neutral:
Ambiguity and Disambiguation - "You know what?"

Japanese source:
バ美肉おじさんになった草wwww
えっwwww高校生じゃないの
English source:
Uncle Bami Meat became Grass
Awww, you are not a student?
MQM annotations:
Major:
Buzzword or Loanword Issues - "Uncle Bami Meat became Grass"
Minor:
no-error
Neutral:
Buzzword or Loanword Issues - "Awww"
Mistranslation - "student"

Japanese source:
昨日ハマスタに行った？
行った！！！！めっちゃスゴなホームランだったな！
English source:
Did you go to Hamasta yesterday?
\zh{You did！！！！ That was a really awesome whole earth hit!}
MQM annotations:
Major:
Dialogue Inconsistency - "You"
Minor:
Terminology or Proper Noun Issues - "Hamasta"
Terminology or Proper Noun Issues - "whole earth hit"
Neutral:
no-error
\end{lstlisting}
}
\caption{The examples used for standard MQM and MQM-Chat automatic annotations few-shots learning.}
\label{fig:few_shots}
\end{figure*}

==> trash/gembamqm_oqs_ec.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[ht]
\centering
\small
\begin{tabular}{@{}lcc@{}}
\toprule
\multicolumn{3}{c}{Chinese $\Rightarrow$ English}  \\ \midrule
                       & \textbf{OQS}   & \textbf{EC}    \\
\textbf{GPT-4 Short }     &   &    \\
\textbf{LLaMA3 Short}     &   &    \\
\textbf{DeepL Short}      &   &    \\
\textbf{Facebook Short}   &   &    \\
\textbf{GPT-4 Long }      &   &    \\
\textbf{LLaMA3 Long}      &   &    \\
\textbf{DeepL Long }      &   &    \\
\textbf{Facebook Long}    &   &    \\  \midrule
\multicolumn{3}{c}{Japanese $\Rightarrow$ English} \\  \midrule
                          & \textbf{OQS}    & \textbf{EC}    \\
\textbf{GPT-4 Short }     &   &    \\
\textbf{LLaMA3 Short}     &   &    \\
\textbf{DeepL Short }     &   &    \\
\textbf{SKIM Short}       &   &   \\
\textbf{GPT-4 Long }      &   &    \\
\textbf{LLaMA3 Long }     &   &    \\
\textbf{DeepL Long }      &   &   \\
\textbf{SKIM Long }       &   &   \\ \bottomrule
\end{tabular}
\caption{The overall quality score (OQS) and total error counts (EC) of translation models based on the standard MQM auto annotations with GEMBA-MQM's prompt.}
\label{tab:gembamqm_oqs_ec}
\end{table}

==> trash/human_severity_heatmap.tex <==
\begin{figure*}[ht]
\centering
%\includegraphics[width=\]
\includegraphics[width=\textwidth]{figure/severity_heatmap.human.pdf}
\caption{The heatmap showing distributions of major, minor, and neutral errors for different error types, across various language pairs and data types.}
\label{fig:severity_heatmap}
\end{figure*}


==> trash/span_overlap_precision_recall_f1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\centering
\small
\begin{tabular}{@{}llllllllll@{}}
\multicolumn{10}{c}{\textit{Chinese-to-English}}                                                                                                                                                                                                                                                                            \\
\multicolumn{1}{c}{}    & \multicolumn{3}{c}{\textbf{Span}}                                                                     & \multicolumn{3}{c}{\textbf{Span-Label}}                                                               & \multicolumn{3}{c}{\textbf{Span-Severity}}                                        \\
\multicolumn{1}{c}{}    & \multicolumn{1}{c}{\textbf{Pre}} & \multicolumn{1}{c}{\textbf{Rec}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{Pre}} & \multicolumn{1}{c}{\textbf{Rec}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{Pre}} & \multicolumn{1}{c}{\textbf{Rec}} & \textbf{F1} \\
\textbf{GPT-4 Short}    & 39.95                            & 49.60                            & 41.00                           & 24.26                            & 25.75                            & 24.26                           & 28.02                            & 31.88                            & 28.28       \\
\textbf{LLaMA3 Short}   & 49.07                            & 60.44                            & 49.83                           & 20.31                            & 23.70                            & 20.36                           & 27.98                            & 33.62                            & 28.28       \\
\textbf{DeepL Short}    & 51.82                            & 63.78                            & 53.67                           & 20.35                            & 22.82                            & 20.37                           & 27.37                            & 33.72                            & 28.66       \\
\textbf{Facebook Short} & 68.13                            & 86.14                            & 71.61                           & 32.13                            & 37.62                            & 32.52                           & 42.03                            & 50.92                            & 43.20       \\
\textbf{GPT-4 Long}     & 23.95                            & 22.83                            & 19.87                           & 14.20                            & 11.70                            & 11.79                           & 12.78                            & 11.01                            & 10.16       \\
\textbf{LLaMA3 Long}    & 27.67                            & 31.39                            & 25.87                           & 12.38                            & 12.98                            & 11.45                           & 14.58                            & 14.97                            & 13.02       \\
\textbf{DeepL Long}     & 41.65                            & 56.93                            & 40.75                           & 13.49                            & 17.00                            & 12.78                           & 16.79                            & 23.60                            & 17.05       \\
\textbf{Facebook Long}  & 42.60                            & 63.08                            & 47.32                           & 16.35                            & 24.49                            & 18.18                           & 22.59                            & 32.97                            & 25.10       \\
\multicolumn{10}{c}{\textit{Japanese-to-English}}                                                                                                                                                                                                                                                                           \\
\multicolumn{1}{c}{}    & \multicolumn{3}{c}{\textbf{Span}}                                                                     & \multicolumn{3}{c}{\textbf{Span-Label}}                                                               & \multicolumn{3}{c}{\textbf{Span-Severity}}                                        \\
\multicolumn{1}{c}{}    & \multicolumn{1}{c}{\textbf{Pre}} & \multicolumn{1}{c}{\textbf{Rec}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{Pre}} & \multicolumn{1}{c}{\textbf{Rec}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{Pre}} & \multicolumn{1}{c}{\textbf{Rec}} & \textbf{F1} \\
\textbf{GPT-4 Short}    & 32.84                            & 29.41                            & 28.42                           & 15.19                            & 13.61                            & 13.64                           & 16.08                            & 14.70                            & 14.41       \\
\textbf{LLaMA3 Short}   & 62.70                            & 40.67                            & 45.49                           & 20.06                            & 14.39                            & 15.38                           & 31.58                            & 20.95                            & 23.38       \\
\textbf{DeepL Short}    & 52.84                            & 45.47                            & 43.11                           & 20.99                            & 16.67                            & 16.69                           & 30.04                            & 23.24                            & 23.36       \\
\textbf{SKIM Short}     & 75.34                            & 53.49                            & 57.59                           & 24.90                            & 18.57                            & 19.40                           & 40.98                            & 29.00                            & 31.03       \\
\textbf{GPT-4 Long}     & \multicolumn{1}{c}{12.13}        & \multicolumn{1}{c}{10.06}        & \multicolumn{1}{c}{9.31}        & \multicolumn{1}{c}{6.75}         & \multicolumn{1}{c}{5.76}         & \multicolumn{1}{c}{5.82}        & \multicolumn{1}{c}{8.28}         & \multicolumn{1}{c}{7.45}         & 7.07        \\
\textbf{LLaMA3 Long}    & \multicolumn{1}{c}{34.13}        & \multicolumn{1}{c}{12.45}        & \multicolumn{1}{c}{16.00}       & \multicolumn{1}{c}{7.61}         & \multicolumn{1}{c}{3.65}         & \multicolumn{1}{c}{4.55}        & \multicolumn{1}{c}{11.70}        & \multicolumn{1}{c}{4.72}         & 5.81        \\
\textbf{DeepL Long}     & \multicolumn{1}{c}{42.89}        & \multicolumn{1}{c}{20.01}        & \multicolumn{1}{c}{24.62}       & \multicolumn{1}{c}{11.37}        & \multicolumn{1}{c}{4.77}         & \multicolumn{1}{c}{6.00}        & \multicolumn{1}{c}{19.41}        & \multicolumn{1}{c}{8.46}         & 10.62       \\
\textbf{SKIM Long}      & 65.82                            & 31.99                            & 39.26                           & 17.29                            & 7.63                             & 9.57                            & 31.35                            & 14.64                            & 18.07      
\end{tabular}
\end{table}
